Towards model based control of the Vertical Gradient Freeze crystal growth process

In this contribution tracking control designs using output feedback are presented for a two-phase Stefan problem arising in the modeling of the Vertical Gradient Freeze process. The two-phase Stefan problem, consisting of two coupled free boundary problems, is a vital part of many crystal growth processes due to the temporally varying extent of the solid and liquid domains during growth. After discussing the special needs of the process, collocated as well as flatness-based state feedback designs are carried out. To render the setup complete, an observer design is performed, using a flatness-based approximation of the original distributed parameter system. The quality of the provided approximations as well as the performance of the open and closed loop control setups is analysed in several simulations.

==> preamble.tex <==
\usepackage[utf8]{inputenc}

% make \vdots and \ddots scale correctly 
% from: https://tex.stackexchange.com/questions/246688/scaling-ddots-in-smallmatrix
\makeatletter
\DeclareRobustCommand\vdots{%
  \mathpalette\@vdots{}%
}
\newcommand*{\@vdots}[2]{%
  % #1: math style
  % #2: unused
  \sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
  \sbox2{$#1.\m@th$}%
  \vbox{%
    \dimen@=\wd0 %
    \advance\dimen@ -3\ht2 %
    \kern.5\dimen@
    % remove side bearings
    \dimen@=\wd2 %
    \advance\dimen@ -\ht2 %
    \dimen2=\wd0 %
    \advance\dimen2 -\dimen@
    \vbox to \dimen2{%
      \offinterlineskip
      \copy2 \vfill\copy2 \vfill\copy2 %
    }%
  }%
}
\DeclareRobustCommand\ddots{%
  \mathinner{%
    \mathpalette\@ddots{}%
    \mkern\thinmuskip
  }%
}
\newcommand*{\@ddots}[2]{%
  % #1: math style
  % #2: unused
  \sbox0{$#1\cdotp\cdotp\cdotp\m@th$}%
  \sbox2{$#1.\m@th$}%
  \vbox{%
    \dimen@=\wd0 %
    \advance\dimen@ -3\ht2 %
    \kern.5\dimen@
    % remove side bearings
    \dimen@=\wd2 %
    \advance\dimen@ -\ht2 %
    \dimen2=\wd0 %
    \advance\dimen2 -\dimen@
    \vbox to \dimen2{%
      \offinterlineskip
      \hbox{$#1\mathpunct{.}\m@th$}%
      \vfill
      \hbox{$#1\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
      \vfill
      \hbox{$#1\mathpunct{\kern\wd2}\mathpunct{\kern\wd2}\mathpunct{.}\m@th$}%
    }%
  }%
}
\makeatother
\usepackage{mathtools}
\newcommand{\svdots}{\raisebox{3pt}{$\scalebox{.75}{$\vdots$}$}}
\newcommand{\sddots}{\raisebox{3pt}{$\scalebox{.75}{$\ddots$}$}} 

% ceil and floor division
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% norm
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

%
\usepackage{booktabs}
\usepackage{tablefootnote}

% gfx
\usepackage{todonotes}
\usepackage{tudcolors}
\usepackage{subcaption}
\usepackage{pgf}
\usepackage{tikz}
\usetikzlibrary{
	shapes,
	arrows.meta,
	bending,
	decorations.markings,
	decorations.pathreplacing,
	decorations.pathmorphing,
	intersections,
	calc,
	positioning,
	external
}
\graphicspath{%
	{res/}%
}

% units
\usepackage[exponent-product=\cdot, tight-spacing=true]{siunitx}

% manage glossaries
\usepackage{glossaries}
\newacronym{dps}{DPS}{distributed parameter system}
\newacronym{bvp}{BVP}{boundary value problem}
\newacronym{fbp}{FBP}{free boundary problem}
\newacronym{sp}{SP}{Stefan problem}
\newacronym{sc}{SC}{Stefan condition}
\newacronym{ode}{ODE}{ordinary differential equation}
\newacronym{pde}{PDE}{partial differential equation}
\newacronym{fem}{FEM}{finite element method}
\newacronym{cfd}{CFD}{computational fluid dynamic}
\newacronym{vgf}{VGF}{Vertical Gradient Freeze}
\newacronym{tmf}{TMF}{travelling magnetic field}
\newacronym{gaas}{GaAs}{Gallium-Arsenide}
\newacronym{inp}{InP}{Indium-Phosphide}
\newacronym{dof}{DOF}{degree of freedom}
\newacronym{iss}{ISS}{Input State Stability}
\newacronym{pi}{CSI}{Poincaré inequality}
\newacronym{csi}{CSI}{Cauchy-Schwarz inequality}
\newacronym{yi}{YI}{Young's inequality}
\newacronym{lti}{LTI}{Linear Time Invartiant}
\newacronym{ltv}{LTV}{Linear Time Vartiant}
\newacronym{lqe}{LQE}{Linear Quadratic Estimator}
\newacronym{frde}{FDRE}{Filtering Riccati Differential Equation}

\usepackage{scrextend}
\usepackage{lineno}
\usepackage[draft]{hyperref}
% Section, Figure, Table always capitalized
\def\sectionautorefname{Section}
\def\subsectionautorefname{Subsection}
\def\figureautorefname{Figure}
\def\tableautorefname{Table}


\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newdefinition{rmk}{Remark}
\newproof{pf}{Proof}
\newproof{pot}{Proof of Theorem \ref{thm2}}

\modulolinenumbers[5]


%%%%%%%%%%%%%%%%%%%%%%%
%% Elsevier bibliography style
%%%%%%%%%%%%%%%%%%%%%%%
%% To change the style, put a % in front of the second line of the current style and
%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%

%% Numbered
%\bibliographystyle{model1-num-names}

%% Numbered without titles
%\bibliographystyle{model1a-num-names}

%% Harvard
%\bibliographystyle{model2-names.bst}\biboptions{authoryear}

%% Vancouver numbered
%\usepackage{numcompress}\bibliographystyle{model3-num-names}

%% Vancouver name/year
%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

%% APA style
%\bibliographystyle{model5-names}\biboptions{authoryear}

%% AMA style
%\usepackage{numcompress}\bibliographystyle{model6-num-names}

%% `Elsevier LaTeX' style
\bibliographystyle{elsarticle-num}
%%%%%%%%%%%%%%%%%%%%%%%

\journal{arXiv.org}

\author[tud]{S. Ecklebe\corref{cor}}
\ead{stefan.ecklebe@tu-dresden.de}
\author[umit]{F. Woittennek}
\ead{frank.woittennek@umit.at}
\author[tud]{J. Winkler}
\ead{jan.winkler@tu-dresden.de}

\author[ikz]{Ch. Frank-Rotsch}
\ead{christiane.frank-rotsch@ikz-berlin.de}
\author[ikz]{N. Dropka}
\ead{natascha.dropka@ikz-berlin.de}

\cortext[cor]{Corresponding author: \texttt{stefan.ecklebe@tu-dresden.de}}
\address[tud]{Institute of Control Theory, Technische Universität Dresden, 01062 Dresden, Germany}
\address[umit]{IACE, Private University for Health Sciences, Medical Informatics and Technology (UMIT), Eduard-Wallnoefer-Zentrum 1, A-6060 Hall in Tirol, Austria}
\address[ikz]{Leibniz Institute for Crystal Growth (IKZ), Max-Born-Str. 2, 12489 Berlin, Germany}



==> simulation.tex <==
\section{A finite dimensional approximation}
\label{sec:fem_model}

\begin{figure}
	\centering
	\def\svgwidth{\linewidth}
	\input{./res/system_annotated_v2.pdf_tex}
	\caption{Schematics of the cylindrical coordinate system $(r, \varphi, z, t)$, a meridional plane (blue)
	and the two domains of the immobilized coordinate $\bar z(t)$.}
	\label{fig:system_v2}
\end{figure}%

Although the feedforward- and control-design in this article series is directly based on the equations
\eqref{eq:lin_heat_eqs} and \eqref{eq:stefan_cond}, for verification of the obtained results,
%simulation purposes
%and observer design 
it is useful to have a finitie dimensional simulation model.
%to approximate the distributed system by
Therefore, this section will introduce a lumped nonlinear state space system of
the form
\begin{equation}
	\xd = f(\x, \uo),\quad \sysout = h(\x)
	\label{eq:nonlin_ss}
\end{equation}
with the initial state $\bs{x}(0) = \bs{x}^0$
% required for a well-posed initial value problem
using the \gls{fem}.
%Note that this represents a set of first order \glspl{ode}, i.e., a finite dimensional system, 
%in contrast to the infinite dimensional system given by \eqref{eq:generic_system}. 
%Consequently, this section derives an approximation of \eqref{eq:generic_system} in the form of \eqref{eq:nonlin_ss}.
%%which will be the basis for the observer design in Section \ref{sec:observer}.

\subsection{Series expansion}
To obtain a finite dimensional approximation, the temperature distribution $T(z,t)$ in each of the
two phases is written as a series
%\footnote{
%	This ansatz
%	%generalized Fourier-Series
%	can be understood as the projection of the infinite dimensional
%	system variable $T(z,t)$ onto a finite dimensional subspace, generated by the shape functions
%	$\varphi_i(z)$.
%}
\begin{equation}
	\toriggz = \lim\limits_{N\to\infty}\sum\limits_{i=1}^N \wbi\varphigz{i}
	\label{eq:gf_series}
\end{equation}
with the time dependent \emph{weights} $\wbi$ and the spatial \emph{shape functions} $\varphigz{i}$
with compact support on $\dom$.
%This is similar to the introduction of the power series in \cite{Ecklebe2018a} used for feedforward control
%design. 
Assuming convergence, the truncation at a certain order $N$ yields the finite-dimensional
approximation
\begin{equation}
	\torigg^N(z,t) = \sum\limits_{i=1}^N \wbi\varphigz{i} \:.
	\label{eq:gf_series_trunc}
\end{equation}
Note that this separation ansatz leaves no option for the shape functions $\varphigz{i}$ to depend
on the time $t$. 
Since the growing crystal and the decrease of melt will alter the spatial domain for both phases
over time it is required to introduce a coordinate transformation in such a way that the  spatial
domain in the transformed system remains constant over the process.
This can be realized by writing the system in new coordinates using a slightly modified version of
the boundary immobilization method as used in \cite{book:AdaptiveMethodofLines, Maidi2014}:
\begin{equation}
	\tfixz = \toriggz \quad \bar z = \frac{z - \zb}{\zbb} \quad \zbb = \zi - \zb \:,
	\label{eq:fix_trafo}
\end{equation}
whose domain is shown on the right-hand side of \autoref{fig:system_v2}.
Thus, yielding\footnote{Details can be found in \autoref{app:trafo_bim}.} two fixed systems
coupled via $\vi$ whose evolution is given by the transformed variant
of the Stefan condition \eqref{eq:stefan_cond}:
\begin{subequations}
	\begin{align}
		\label{eq:fixiated_heat_eq_pde}
		\partial_t \tfixz &= \frac{\hd}{\zbbsq}\partial_{\bar z}^2\tfixz
		+ \frac{\bar z \vi}{\zbb} \partial_{\bar z} \tfixz \\
		\label{eq:fixiated_heat_eq_bc1}
		\hc\partial_{\bar z} \tfix(0, t) &= \bfd\zbb\inp \\
		\label{eq:fixiated_heat_eq_bc2}
		\tfix(1, t) &= \tm \\
		\vi &= \frac{1}{L\dmelt} \Bigg[
			\frac{\hcs}{\zbbs}\partial_{\bar z}\tfixs(1, t)
			-\frac{\hcl}{\zbbl}\tfixl(1, t)
		\Bigg] \:.
	\label{eq:fixiated_stefan_cond}
\end{align}
	\label{eq:fixiated_heat_eq}%
\end{subequations}%
Now, the approximation of the series expansion \eqref{eq:gf_series_trunc} can be expressed in the transformed
coordinates
\begin{equation}
	\tappz = \sum\limits_{i=1}^N \wbi\varphibgz{i}
	\label{eq:gf_series_fixed}
\end{equation} %jcw: nachfolgenden Absatz ggf. noch präzisieren
with the shape functions $\varphibgz{i} \in C^0_{\textup{c}}(0, 1)$, $i=1,\dotsc,N$.
Note that herein only one set of shape functions
%$\varphibgz{i}, i=1,\dotsc,N$
is be utilised for both phases due to their consistent domains.
For the approximation, piecewise-linear basis functions with the spatial discretisation
$\dzb = \frac{1}{N-1}$, are used.
In detail, they are given by
%\begin{align}%
%	\varphi_{i}(z) &= \begin{cases}
%		\varphi_i^{\left\{1\right\}}(z)\quad &\text{für } z \in \left(z_{i-1}, z_{i}\right] \\
%		\varphi_i^{\left\{2\right\}}(z)\quad &\text{für } z \in \left(z_{i}, z_{i+1}\right) \\
%		0 \quad\text{sonst,}
%		\end{cases} 
%	\label{eq:swm_fem_lag1st}
%    \intertext{mit den Geradenfunktionen} %$\varphi_i^{\left\{1\right\}}(z)$ und $\varphi_i^{\left\{2\right\}}(z)$
%	\varphi_i^{\left\{1\right\}}(z) &= \frac{z - z_{i-1}}{\Delta z}\:\text{und }\
%	\varphi_i^{\left\{2\right\}}(z) = -\frac{z - z_{i+1}}{\Delta z} \:.
%	\label{eq:swm_fem_lag1st_local}
%\end{align}
\begin{subequations}
	\begin{align}
		\varphibgz{i} &= \begin{cases}
			\frac{\bar z - (i - 1)\dzb}{\dzb} &\text{for } (i - 1)\dzb < \bar z \le i\dzb\\
			\frac{\bar z - (i + 1)\dzb}{\dzb} &\text{for } i\dzb < \bar z < (i+1)\dzb\\
			0 & \text{otherwise}
		\end{cases}
		\label{eq:lag1st_center}
		\intertext{for the general case $i \not\in \left\{1, N\right\}$ and}
		\varphibgz{1} &= \begin{cases}
			\frac{\bar z - 2\dzb}{\dzb} &\text{for } 0 < \bar z < \dzb\\
			0 & \text{otherwise}
		\end{cases}
		\label{eq:lag1st_left}
		\intertext{as well as}
		\varphibgz{N} &= \begin{cases}
			\frac{\bar z - (N - 1)\dzb}{\dzb} &\text{for } (N - 1)\dzb < \bar z \le 1\\
			0 & \text{otherwise}
		\end{cases}
		\label{eq:lag1st_right}
	\end{align}%
	\label{eq:lag1st}%
\end{subequations}%
at the outer and inner boundary, respectively.
%depicted in upper part of \autoref{fig:lag1st},
Hence, the Dirichlet boundary condition \eqref{eq:fixiated_heat_eq_bc2} directly evaluates to 
$\wb_N(t) = \tm$, since only $\bar\varphi^N_N(\bar z)$ differs from zero at $\bar z = 1$.
This motivates a choice of $N \ge 2$.

\subsection{Projection}
By choosing a Galerkin ansatz, \eqref{eq:fixiated_heat_eq_pde} is projected on the remaining
set of $N-1$ functions, yielding equations of the form
\begin{align}
	\begin{split}
		\inner{\partial_t \tappz}{\varphibgz{k}}
		&= \frac{\hd}{\zbbsq}\inner{\partial_{\bar z}^2\tappz}{\varphibgz{k}}\\
		&\hphantom{=}+ \frac{\vi}{\zbb}\inner{\bar z \partial_{\bar z} \tappz}{\varphibgz{k}}
	\end{split}
	\label{eq:fixiated_heat_eq_weak_1}
\end{align}
for $k = 1,\dotsc,N-1$.
Herein, $\inner{\zeta(z)}{\psi(z)} = \int_\Omega \zeta(z)\psi(z)\,\textup{d}z$ denotes the standard 
inner product on $L_2$ for real-valued arguments.
Performing integration by parts on the first right-hand side term of \eqref{eq:fixiated_heat_eq_weak_1}
eventually delivers the weak form
\begin{align}
	\begin{split}
		\inner{\partial_t \tfixz}{\varphibgz{k}}
		&= \frac{\hd}{\zbbsq}\bigg(
			\left[\partial_{\bar z}\tfixz \varphibgz{k}\right]_0^1 \\
		&\hphantom{=\frac{\hd}{\zbbsq}\bigg(}	-\inner{\partial_{\bar z}\tfixz}{\partial_{\bar z}\varphibgz{k}}
			\bigg)\\
		&\hphantom{=}+ \frac{\vi}{\zbb}\inner{\bar z \partial_{\bar z} \tfixz}{\varphibgz{k}}
	\end{split}
	\label{eq:fixiated_heat_eq_weak_2}
\end{align}
of the problem for each $\varphibgz{k}$ $k=1,\dotsc, N-1$.
Utilising the boundary conditions \eqref{eq:fixiated_heat_eq_bc1} and \eqref{eq:fixiated_heat_eq_bc2},  
by introducing the vector of the remaining free variables 
$\wbv = \begin{pmatrix}
	\wb_{\bullet,1}(t), \dotsc, \wb_{\bullet,N-1}(t)
\end{pmatrix}^T$, 
all $N-1$ equations from \eqref{eq:fixiated_heat_eq_weak_2} can be combined using a matrix-vector notation:
\begin{align}
	\wbvt =&
	-\frac{\hd}{\zbbsq} \bs{P}_{0,0}^{-1}\Big(
		\bs{P}_{1,1}\wbv
		+ \bs{q}_{1,1}\tm
		\nonumber\\
		&\quad\qquad
		+\frac{\bfd}{\hc}\zbb\inp \bar{\bs{\varphi}}^N_0
	\Big) \nonumber\\
	&+ \frac{\vi}{\zbb} \bs{P}_{0, 0}^{-1} \left(
		\bs{P}_{1,0} \wbv
		+ \bs{q}_{1,0}\tm
	\right) \:.
	\label{eq:gen_ode_sys}
\end{align}
Herein, the matrices $\bs{P} \in \mathbb{R}^{(N-1)\times(N-1)}$ and vectors 
$\bs{q} \in \mathbb{R}^{(N-1)\times 1}$ contain the various inner products\footnote{
The resulting expressions for coefficient vectors and matrices are given in \ref{app:b}.},
while the shape functions evaluated at zero are given by the vector
$\bar{\bs{\varphi}}^N_0 = \begin{pmatrix} \bar\varphi^N_1(0), \dotsc, \bar\varphi^N_{N-1}(0)
\end{pmatrix}^T$.
%Note that this system of \glspl{ode} is valid for both phases with only one set of
%shape functions $\varphibgz{i}$,
%just by replacing the generic parameters with their solid and liquid counterparts.
Thus, \gls{ode} systems for the weights of the solid and liquid phase
-- given by $\wbvs$ and $\wbvl$, respectively --
are obtained.
Writing \eqref{eq:fixiated_stefan_cond} in the new variables yields:
\begin{align}
	\begin{split}
		\vi &= \frac{1}{L\dmelt} \Bigg[
			\frac{\hcs}{\zbbs} \Big(
				\bar{\bs{\varphi}}^{N'}_1 \wbvs
				+ \bar{\varphi}^{N'}_N(1) \tm
			\Big)\\
			&\qquad\qquad-\frac{\hcl}{\zbbl}\Big(
				\bar{\bs{\varphi}}^{N'}_1 \wbvl
				+ \bar{\varphi}^{N'}_N(1) \tm
			\Big)
		\Bigg] \:.
	\end{split}
	\label{eq:fixiated_stefan_cond_approx}
\end{align}
Therein,
$\bar{\bs{\varphi}}^{N'}_1 = \begin{pmatrix}
	\partial_{\bar z} \bar\varphi^N_1(1), \dotsc, \partial_{\bar z} \bar\varphi^N_{N-1}(1)
\end{pmatrix}^T$.

In order to make the derived system compatible with the general state space formulation
\begin{equation*}
	\xd = f(\x, \uo),\quad \sysout = h(\x)
\end{equation*}
from \eqref{eq:nonlin_ss}, firstly, the state vector
\begin{equation}
	\bs{x}^N(t) := \begin{pmatrix}
		\bar{\bs{w}}_{\textup{s}}^{N^T}(t), \bar{\bs{w}}_{\textup{l}}^{N^T}(t), \zi
\end{pmatrix}^T \in \mathbb{R}^M  \label{eq:state_vector}
\end{equation}
where $M = 2(N-1) + 1$, is introduced. Note that due to the incorporation of 
\eqref{eq:fixiated_stefan_cond}, the interface position $\zi$ explicitly appears as a state variable.
Secondly, the heater powers are collected in the input vector
$\uo := \begin{pmatrix}
	\inps, \inpl
\end{pmatrix}^T$.
Thirdly, the measurable system output $\sysout[fem]$ is given by the boundary temperatures
$\tapp(\zb, t)$, 
which can be directly expressed by their corresponding weights, yielding
\begin{equation}
	\sysout[fem] = \outmap{fem}{\bs{x}^N(t)} = \begin{pmatrix}
		\wb_{\mathrm{s},0}(t), \wb_{\mathrm{l},0}(t)
	\end{pmatrix}^T
\end{equation}
due to the special choice of the shape functions $\bar \varphi^N_i(\bar z)$.
Finally, the initial state 
%$\bs{x}^0 = \bs{x}(0)$
of the system is given by
\begin{equation}
	\bs{x}^N(0) = \begin{pmatrix}
		\bar{\bs{w}}_{\textup{s}}^{N^T}(0), \bar{\bs{w}}_{\textup{l}}^{N^T}(0), \gamma(0)
	\end{pmatrix}^T.
\end{equation}
Herein, the weights for the solid or liquid phase $\bar{\bs{w}}_{i,\textup{s}}(0)$ are obtained 
by the projection
\begin{equation}
	\wb_{\bullet,i}(0) = \inner{\bar\varphi^N_i(\bar z)}{\tfix(\bar z, 0}, \quad i=1,\dotsc,N-1
	\label{eq:initial_weights}
\end{equation}
of the respective initial temperature profile onto the shape functions $\varphibgz{i}$.

%The resulting projection of an exemplary function is illustrated in the bottom half of \autoref{fig:lag1st}.
%\begin{figure}
%	\centering
%	\resizebox {\linewidth} {!} {
%		\input{./res/lag1st_proj.pgf}
%	}
%	\caption{A set of $N=4$ Lagrangian basis functions $\bar\varphi^N_i(\bar z)$ of order one (top) and the 
%		projection $\tilde g(\bar z)$ (solid, dark) of an exemplary function $g(\bar z)$ (dashed, light),
%		using the approximation weights $\bar w_i$ (bottom).
%	}
%	\label{fig:lag1st}
%\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "article"
%%% End:

